Constructing segments of quadratic length in $Spec(T_n)$ through segments of linear length

A Transposition graph $T_n$ is defined as a Cayley graph over the symmetric group $Sym_n$ generated by all transpositions. It is known that the spectrum of $T_n$ consists of integers, but it is not known exactly how these numbers are distributed. In this paper we prove that integers from the segment $[-n, n]$ lie in the spectrum of $T_n$ for any $n\geqslant 31$. Using this fact we also prove the main result of this paper that a segment of quadratic length with respect to $n$ lies in the spectrum of $T_n$.

==> table.tex <==

\setlength{\arrayrulewidth}{0.1mm}
\setlength{\tabcolsep}{2pt}
\renewcommand{\arraystretch}{2}


\begin{table}[!h]
    \centering
   \begin{tabular}{ |c|c|c|c| } 
\hline
Eigenvalues, $\lambda$ & Partitions & Limitations & Proof  \\
\hline

$\frac{n + 3}{2} \leqslant \lambda \leqslant n - 4$ & $(\frac{\lambda}{2} + \frac{3}{2}, \frac{n + 2}{2} - \frac{\lambda}{2}, 3, 2\times(\frac{n-4}{2} - \frac{\lambda}{2}), 1\times (\lambda - \frac{n + 3}{2}))$ & $\lambda \ is \ odd, n \ is \ odd$ & 
\\
\hline
$\frac{n+7}{2} \leqslant \lambda \leqslant n - 7$ & $(\frac{\lambda}{2}, \frac{n+3}{2} - \frac{\lambda}{2}, 5,
2\times(\frac{n-3}{2} - \frac{\lambda}{2}), 1\times(\lambda -\frac{n + 7}{2}))$ & $\lambda \ is \ even, \ n \ is \ odd$ &
\\
\hline
$\frac{n+4}{2} \leqslant \lambda \leqslant n - 1$ & $(\frac{\lambda}{2}+\frac{3}{2}, \frac{n+3}{2}-\frac{\lambda}{2},2, 2\times(\frac{n-3}{2}-\frac{\lambda}{2}), 1 \times (\lambda - \frac{n+4}{2}))$ & $\lambda \ is \ odd, \ n \ is \ even$ &
\\
\hline
$\frac{n+4}{2} \leqslant \lambda \leqslant n - 6$&$(\frac{\lambda}{2}+\frac{2}{2}, \frac{n+2}{2}-\frac{\lambda}{2}, 4,  2\times(\frac{n-4}{2}-\frac{\lambda}{2}), 1 \times (\lambda - \frac{n+4}{2}))$ & $\lambda \ is \ even, \ n \ is \ even$ &
\\
\hline
\end{tabular}  
    \caption{ \label{main-table}  Summary of the technical lemmas.}
\end{table}





\begin{table}[!h]

\begin{tabular}{|c|c|c|}
	\hline
	Eigenvalue, $\lambda$ & Partitions  & Parity of $n$\\
	\hline
 \begin{tabular}{c} 
 $\frac{n+1}{2}$ \\ $\frac{n+3}{2}$ \\ $\frac{n+5}{2}$
 \end{tabular} & \begin{tabular}{c}
      $(\frac{n-11}2, 7, 4,3,3, 1\times(\frac{n-23}2))$
      \\ $(\frac{n-1}2, 4, 1\times(\frac{n-7}2))$ 
      \\ $(\frac{n-3}2, 5, 2, 1\times(\frac{n-11}2))$
 \end{tabular} & odd
\\
\hline
\begin{tabular}{c} 
 $\frac{n-2}{2}$ \\ $\frac{n}{2}$ \\ $\frac{n+2}{2}$
 \end{tabular} & \begin{tabular}{c}
      $(\frac{n-16}2, 8, 5, 4, 3, 3, 1\times(\frac{n-30}2))$
      \\ $(\frac{n+2}2, 1\times(\frac{n-2}2))$ 
      \\ $(\frac{n-12}2, 8, 3, 3, 3, 2, 1\times(\frac{n-26}2))$
 \end{tabular} & even
\\
\hline
	\end{tabular}	
    \caption{ \label{main-table}  Summary of the technical lemmas.}
 \end{table}


\begin{table}[!h]

\begin{tabular}{|c|c|}
	\hline
	Eigenvalue, $\lambda$ & Partitions \\
	\hline
 \begin{tabular}{c} 
 $n$
 \end{tabular} 
 & \begin{tabular}{c}
      $(\frac{n+3}2, 1\times(\frac{n-3}2))$
      \\ $(\frac{n}2, 4, 1\times(\frac{n}2-4))$ 
 \end{tabular}
 \\
 \hline
  \begin{tabular}{c} 
 $n-1$
 \end{tabular} 
 & \begin{tabular}{c}
      $(\frac{n+1}2,3, 1\times(\frac{n-7}2))$
      \\ $(\frac{n+2}2,2, 1\times(\frac{n}2 - 3))$ 
 \end{tabular}
  \\
 \hline
  \begin{tabular}{c} 
 $n-2$
 \end{tabular} 
 & \begin{tabular}{c}
      $(\frac{n-1}2,4, 2, 1\times(\frac{n-11}2))$
      \\ $(\frac{n-8}2, 6, 5, 3, 1\times(\frac{n}2 - 10))$ 
 \end{tabular}
\\
 \hline
  \begin{tabular}{c} 
 $n-3$
 \end{tabular} 
 & \begin{tabular}{c}
      $(\frac{n+1}2, 2, 2, 1\times(\frac{n-9}2))$
      \\ $(\frac{n}2, 3, 2, 1\times(\frac{n-10}2))$ 
 \end{tabular}
 \\
 \hline
  \begin{tabular}{c} 
 $n-4$
 \end{tabular} 
 & \begin{tabular}{c}
      $(\frac{n-1}2, 3, 3, 1\times(\frac{n-11}2))$
      \\ $(\frac{n-4}2, 5, 3, 2, 1\times(\frac{n-16}2))$ 
 \end{tabular}
  \\
 \hline
  \begin{tabular}{c} 
 $n-5$
 \end{tabular} 
 & \begin{tabular}{c}
      $(\frac{n-7}2, 5, 5, 3, 1\times(\frac{n-19}2))$
      \\ $(\frac{n-2}2, 4, 2, 2, 1\times(\frac{n-14}2))$ 
 \end{tabular}
  \\
 \hline
  \begin{tabular}{c} 
 $n-6$
 \end{tabular} 
 & \begin{tabular}{c}
      $(\frac{n-1}2, 3, 2, 2, 1\times(\frac{n-13}2))$
      \\ $(\frac{n}2, 2, 2, 2, 1\times(\frac{n-12}2))$ 
 \end{tabular}
 \\
 \hline
\end{tabular}	
\caption{ \label{main-table}  Summary of the technical lemmas.}
\end{table}


% \begin{sidewaystable}[!h]
%     \centering



% \begin{sidewaystable}[!h]
% \centering
% \begin{tabular}{|c|c|c|c|c|c|c|c|}
% 	\hline
% 	& $n$ & $n-1$ & $n-2$ & $n-3$ & $n-4$ & $n-5$ & $n-6$ \\
  
% 	\hline
%  $odd$ & $(\frac{n+3}2, 1\times(\frac{n-3}2))$ & $(\frac{n+1}2,3, 1\times(\frac{n-7}2))$ & $(\frac{n-1}2,4, 2, 1\times(\frac{n-11}2))$
%  & $(\frac{n+1}2, 2, 2, 1\times(\frac{n-9}2))$ & $(\frac{n-1}2, 3, 3, 1\times(\frac{n-11}2))$ & $(\frac{n-7}2, 5, 5, 3, 1\times(\frac{n-19}2))$
%  &  $(\frac{n-1}2, 3, 2, 2, 1\times(\frac{n-13}2))$ \\
%  \hline
%  $even$ & $(\frac{n}2, 4, 1\times(\frac{n}2-4))$ & $(\frac{n+2}2,2, 1\times(\frac{n}2 - 3))$ & $(\frac{n-8}2, 6, 5, 3, 1\times(\frac{n}2 - 10))$ & $(\frac{n}2, 3, 2, 1\times(\frac{n-10}2))$ &
%  $(\frac{n-4}2, 5, 3, 2, 1\times(\frac{n-16}2))$ & $(\frac{n-2}2, 4, 2, 2, 1\times(\frac{n-14}2))$ & $(\frac{n}2, 2, 2, 2, 1\times(\frac{n-12}2))$  \\
%  \hline
 
%  \end{tabular}	
% \caption{ \label{main-table}  Summary of the technical lemmas.}
% \end{sidewaystable}




%  \begin{tabular}{c} 
%  $n$
%  \end{tabular} 
%  & \begin{tabular}{c}
%       $(\frac{n+3}2, 1\times(\frac{n-3}2))$
%       \\ $(\frac{n}2, 4, 1\times(\frac{n}2-4))$ 
%  \end{tabular}
%  \\
%  \hline
%   \begin{tabular}{c} 
%  $n-1$
%  \end{tabular} 
%  & \begin{tabular}{c}
%       $(\frac{n+1}2,3, 1\times(\frac{n-7}2))$
%       \\ $(\frac{n+2}2,2, 1\times(\frac{n}2 - 3))$ 
%  \end{tabular}
%   \\
%  \hline
%   \begin{tabular}{c} 
%  $n-2$
%  \end{tabular} 
%  & \begin{tabular}{c}
%       $(\frac{n-1}2,4, 2, 1\times(\frac{n-11}2))$
%       \\ $(\frac{n-8}2, 6, 5, 3, 1\times(\frac{n}2 - 10))$ 
%  \end{tabular}
% \\
%  \hline
%   \begin{tabular}{c} 
%  $n-3$
%  \end{tabular} 
%  & \begin{tabular}{c}
%       $(\frac{n+1}2, 2, 2, 1\times(\frac{n-9}2))$
%       \\ $(\frac{n}2, 3, 2, 1\times(\frac{n-10}2))$ 
%  \end{tabular}
%  \\
%  \hline
%   \begin{tabular}{c} 
%  $n-4$
%  \end{tabular} 
%  & \begin{tabular}{c}
%       $(\frac{n-1}2, 3, 3, 1\times(\frac{n-11}2))$
%       \\ $(\frac{n-4}2, 5, 3, 2, 1\times(\frac{n-16}2))$ 
%  \end{tabular}
%   \\
%  \hline
%   \begin{tabular}{c} 
%  $n-5$
%  \end{tabular} 
%  & \begin{tabular}{c}
%       $(\frac{n-7}2, 5, 5, 3, 1\times(\frac{n-19}2))$
%       \\ $(\frac{n-2}2, 4, 2, 2, 1\times(\frac{n-14}2))$ 
%  \end{tabular}
%   \\
%  \hline
%   \begin{tabular}{c} 
%  $n-6$
%  \end{tabular} 
%  & \begin{tabular}{c}
%       $(\frac{n-1}2, 3, 2, 2, 1\times(\frac{n-13}2))$
%       \\ $(\frac{n}2, 2, 2, 2, 1\times(\frac{n-12}2))$ 
%  \end{tabular}
%  \\
%  \hline
% \end{tabular}	
% \caption{ \label{main-table}  Summary of the technical lemmas.}
% \end{table}
